Region-Aware Diffusion for Zero-shot Text-driven Image Editing

Image manipulation under the guidance of textual descriptions has recently received a broad range of attention. In this study, we focus on the regional editing of images with the guidance of given text prompts. Different from current mask-based image editing methods, we propose a novel region-aware diffusion model (RDM) for entity-level image editing, which could automatically locate the region of interest and replace it following given text prompts. To strike a balance between image fidelity and inference speed, we design the intensive diffusion pipeline by combing latent space diffusion and enhanced directional guidance. In addition, to preserve image content in non-edited regions, we introduce regional-aware entity editing to modify the region of interest and preserve the out-of-interest region. We validate the proposed RDM beyond the baseline methods through extensive qualitative and quantitative experiments. The results show that RDM outperforms the previous approaches in terms of visual quality, overall harmonization, non-editing region content preservation, and text-image semantic consistency. The codes are available at https://github.com/haha-lisa/RDM-Region-Aware-Diffusion-Model.

==> Figures/teaser.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{Images/teaser5}
%     % \vspace{-0.2cm} 
%     \caption{The outputs of Diff-Edit manipulation. The texts adhere to the phrase rule "A → B", indicating that Diff-Edit transforms entity A into entity B.}
%     % \vspace{-0.4cm} 
%     \label{fig:teaser}
% \end{figure*}

% \begin{teaserfigure}
%     \includegraphics[width=\textwidth]{Images/teaser5}
%     \caption{The results of the proposed region-aware diffusion model (RDM). The texts adhere to the phrase rule ``A → B'', indicating that RDM transforms entity A into entity B.}
%     % \Description{figure description}
%     \label{fig:teaser}
% \end{teaserfigure}

==> Sections/1_bak.tex <==
\section{Introduction}
%----------------------------------paragraph 1-------------------------------------
%1
In the actual world, image editing is highly sought-after.
%2
However, image content editing software is not easy to get started with and is more suited to professionals.
%3
Present image editing work is limited in terms of possible input images and editing operations.
%4
In recent years, great advances in deep generative image models~\cite{vqgan, Guided-Diffusion, latentdiffusion} and visual language pre-training models~\cite{clip} have made text-based image generation and manipulation interfaces possible.

%----------------------------------paragraph 2-------------------------------------
%1
There are different principal branches of image generation, such as inpainting, image translation~\cite{choi2021ilvr}, style transfer~\cite{huang2017arbitrary} and image manipulation~\cite{wang2022manitrans, nichol2021glide, ramesh2022hierarchical, avrahami2022blended, avrahami2022latentblended}. 
%2
Computational approaches~\cite{openedit, bau2021paint, Flexit_2022_CVPR} for modifying the style and appearance of objects in natural photographs have made remarkable progress, allowing beginner users to accomplish a wide range of editing effects.
%3
Nevertheless, it should be noted that prior text image manipulations work either did not allow for arbitrary text commands or image manipulation~\cite{mo2018instagan, bau2021paint, diffusionCLIP_2022_CVPR} or only allowed for modifications to the image's appearance properties or style~\cite{openedit, jiang2021language}.
%4
Controlling the localization of modifications normally requires the user to draw a region to specify~\cite{avrahami2022blended, avrahami2022latentblended, bau2021paint}, which adds to the complexity of the operation.
%5
In this study, we aim to eliminate all of the aforementioned constraints and restrictions in order to enable open image content modification with pure textual control utilizing cutting-edge image generation techniques.

%----------------------------------paragraph 3-----------------------------------
%1
Recently, there have been tremendous advances in multimodal deep learning that have opened the way for machines to achieve cross-modal communication and control.
%2
One of the large-scale multimodal pre-training models that have received many applications is the Contrastive Language Image Pretraining(CLIP)~\cite{clip} model, which was pre-trained on 400 million text-image samples.
%3
In parallel, various new image synthesis methods~\cite{StyleCLIP, StyleGANNADA, CLIPstyler, kim2021diffusionclip, ramesh2022hierarchical, Huang2022MGAD} have highlighted the richness of the vast visual and linguistic realm encompassed by CLIP.
%4
Nonetheless, manipulating existing items in arbitrary, actual pictures continues to remain tricky.
%5
The present mainstream techniques combine CLIP with pre-trained GANs generators, however, the input picture domain is constrained.
%6
There has recently been a tremendous amount of interest in diffusion models, which generate high-quality, diversified pictures.
%7
Image manipulation at the pixel level, on the other hand, leads to extended generation times and excessive computer resource consumption.



%----------------------------------paragraph 4--------------------------------------
%1
After investigation, we found that applying the diffusion process in the latent space of pre-trained autoencoders~\cite{latentdiffusion} can speed up inference and reduce the consumption of computational resources.
%2
Nevertheless, previous latent diffusion models still fall short in terms of generating image realism. 
To improve image realism and to enhance the consistency of the editing results with the guide text, we introduced classifier-free guidance~\cite{ho2021classifier} at each step of the diffusion.
%3
Based on these, we develop an intensive high-performance diffusion model editing (Diff-Edit) framework for zero-shot text-driven image editing.
%4
Specifically, our method enables the editing of image content that satisfies an arbitrary given text prompt (as shown in Fig.~\ref{fig:teaser}). 
%5
For example, given an image of the dog, and the positioning text: "A dog", our work can position the corresponding editing area. 
%6
Then, based on the target text: "A cat", a high-quality, realistic, and varied image can finally be composed.

%----------------------------------paragraph 5--------------------------------------
%1
To enables the user to specify the area and objects to be modified and the objects to be created, simply and intuitively, we present a cross-modal entity calibration component. %2
It can locate and adjust the text-relevant picture tokens given the positional textual guidance $t_1$ to correctly identify the entities for modification.
%3
We observed that by feeding the input image into the encoder together with the mask, the content outside of the mask appeared transformed in an unexpected way during the diffusion process for image modification.
To retain extraneous content to a greater extent, we perform further diffusion at each diffusion step where it blends the clip-guided diffusion result with the corresponding noisy version of the input image.
In addition, we build relevant loss functions that protect non-editing domains to constrain the generative process.
%4
We incorporated the clip gradient into the classifier-free guidance to make the edited results more favorable to humans and to make the content generated in the edit area more consistent with the semantic content of the target textual guidance $t_2$.
%5
Overall, Diff-Edit implements enhanced directional guidance in the latent space to generate rapid, high-quality, realistic, and text-compliant editing results.



%----------------------------------paragraph 6--------------------------------------
%1
Quantitative and qualitative comparisons with previous approaches reveal that our method can better manipulate the entities of an image through text while leaving the background region unaffected. 
%2
As shown in Figs.~\ref{fig:teaser},~\ref{fig:moreresults2} and \ref{fig:moreresults1}, 
Diff-Edit is capable of producing realistic and high-quality outcomes in terms of object content change when guided by various image inputs and text descriptions.
%3
The main contributions of this work are summarized as follows:
\begin{itemize}
\item We propose Diff-Edit, an entity-level zero-shot text-driven image editing framework based on the intensive diffusion model.
\item We introduced spatial location masks into each step of the diffusion sampling and created non-editing domain preserving loss functions to obtain edited results without stitching traces and well-preserved unedited regions.
\item We manipulate the diffusion step in latent space and embed enhanced directional guidance structures to enhance image realism and improve the consistency of the control text with the editing result.
\item The quantitative and qualitative experimental results show that Diff-Edit outperforms baseline methods in terms of quality, veracity, and diversity in text-guided image editing, and achieves superior results.
\end{itemize}

==> Tables/userstudy.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[htbp]
  \centering
    \caption{User study results. Each number represents the percentage of votes received by the other models' outcomes as compared to our results.}
    \begin{tabular}{rccccc}
    \toprule
                &             & Latent diffusion  & GLIDE       & Blended diffusion & CLIP guided diffusion \\
    \midrule
                & Visual quality & 5.71\%      & 19.05\%     & 6.67\%      & 15.71\% \\
    \multicolumn{1}{c}{Preference rate} & Invisible seams & 6.67\%      & 20.95\%     & 10.00\%     & 16.67\% \\
                & Text consistency & 10.48\%     & 24.29\%     & 21.43\%     & 11.90\% \\
    \bottomrule
    \end{tabular}%
  \vspace{+0.4cm}
  \label{tab:userstudy}%
\end{table*}%
